Towards Understanding the Benefit of Multitask Representation Learning in Decision Process

Multitask Representation Learning (MRL) has emerged as a prevalent technique to improve sample efficiency in Reinforcement Learning (RL). Empirical studies have found that training agents on multiple tasks simultaneously within online and transfer learning environments can greatly improve efficiency. Despite its popularity, a comprehensive theoretical framework that elucidates its operational efficacy remains incomplete. Prior analyses have predominantly assumed that agents either possess a pre-known representation function or utilize functions from a linear class, where both are impractical. The complexity of real-world applications typically requires the use of sophisticated, non-linear functions such as neural networks as representation function, which are not pre-existing but must be learned. Our work tries to fill the gap by extending the analysis to \textit{unknown non-linear} representations, giving a comprehensive analysis for its mechanism in online and transfer learning setting. We consider the setting that an agent simultaneously playing $M$ contextual bandits (or MDPs), developing a shared representation function $\phi$ from a non-linear function class $\Phi$ using our novel Generalized Functional Upper Confidence Bound algorithm (GFUCB). We formally prove that this approach yields a regret upper bound that outperforms the lower bound associated with learning $M$ separate tasks, marking the first demonstration of MRL's efficacy in a general function class. This framework also explains the contribution of representations to transfer learning when faced with new, yet related tasks, and identifies key conditions for successful transfer. Empirical experiments further corroborate our theoretical findings.

==> cov_letter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Manuscript Title}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies \red{X, Y, and Z} which is important because of \red{A, B, and C}.

This paper extends our work of \red{Conference Paper} by addressing \red{X, Y, and Z additional points}.

We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}

Our submission has the following keywords: \red{keyword}, \red{keyword}, \red{keyword}, \red{keyword}, \red{keyword}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Co-Author (Institution)}\\
\red{Co-Author (Institution)}\\
\red{Co-Author (Institution)}\\
\red{Co-Author (Institution)}

\end{document}







































